Cost Control and Efficiency Optimization in Maintainability Implementation of Wireless Sensor Networks based on Serverless Computing

Wireless sensor network (WSN) has been developed for decades and have performed well in the performance, power consumption, and congestion control. However, the following problems have not been addressed, such as inaccurate cost estimation of device's lifecycle, highly-coupled engineering development, and low utilization of hardware and software resources during the life cycle of WSN. Therefore, we first propose the conceptual view of maintainability implementation for WSN based on Serverless Computing. The maintainability implementation refers to the ability to meet the WSN product to consume the minimum resources with a higher probability in configuration, trial production, debugging, batch production, deployment, operation, and maintenance phases. And then, we discuss that Serverless Computing can be realized at the software functional level of WSN to decouple the device operation and functional development, greatly improve the reuse of resources and exclude the hardware interference. From the perspective of maintainability and cost control, the concept of Serverless Computing can be used to build WSN platforms, which can support the functions of data collection and data management into functional development that may benefit from exploration through upfront expenditures, thereby significantly reducing design, manufacturing, and operational costs. Finally, based on existing technologies and smart city scenarios, the idea of a WSN platform for Serverless Computing is given with a case study.

==> author/references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%


\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% % Contribution 
% \bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
% %
% % Online Document
% \bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
% \url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
% %
% % Monograph
% \bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
% %
% % Journal article
% \bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
% %
% % Journal article by DOI
% \bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
% %
% \bigskip

% % Use the following (APS) syntax and markup for your references if 
% % the subject of your book is from the field 
% % "Mathematics, Physics, Statistics, Computer Science"
% %
% % Online Document
% \bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
% \url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
% %
% % Monograph
% \bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
% %
% % Journal article
% \bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
% %
% % Journal article by DOI
% \bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
% %
% % Contribution 
% \bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
% %
% \bigskip
% %
% % Use the following syntax and markup for your references if 
% % the subject of your book is from the field 
% % "Psychology, Social Sciences"
% %
% %
% % Monograph
% \bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
% %
% % Online Document
% \bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
% \url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
% %
% % Journal article
% \bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
% %
% % Contribution 
% \bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
% %
% % Journal article by DOI
% \bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
% %
% %
% % Use the following syntax and markup for your references if 
% % the subject of your book is from the field 
% % "Humanities, Linguistics, Philosophy"
% %
% \bigskip
% %
% % Journal article
% \bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
% %
% % Contribution 
% \bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
% %
% % Monograph
% \bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
% %
% % Online Document
% \bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
% http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
% %
% % Journal article by DOI
% \bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
% %
% %
% %
% \bigskip
% %
% %
% % Use the following syntax and markup for your references if 
% % the subject of your book is from the field 
% % "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
% %
% %
% % Contribution 
% \bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
% %
% % Online Document
% \bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
% \url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
% %
% % Journal article by DOI
% \bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
% %
% % Journal article
% \bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
% %
% % Monograph
% \bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
% %

\bibitem{MEMS-acm} G. Vasanthi and N. Prabakaran. 2022. An improved approach for energy consumption minimizing in WSN using Harris hawks optimization. J. Intell. Fuzzy Syst. 43, 4 (2022), 4445–4456. https://doi.org/10.3233/JIFS-213252

\bibitem{sync-proto-survey-acm} Zimmerling M, Mottola L, Santini S. Synchronous transmissions in low-power wireless: A survey of communication protocols and network services[J]. ACM Computing Surveys (CSUR), 2020, 53(6): 1-39.

\bibitem{isac-limit} A. Liu et al., “A Survey on Fundamental Limits of Integrated Sensing and Communication,” IEEE Commun. Surv. Tutorials, vol. 24, no. 2, pp. 994–1034, 2022, doi: 10.1109/COMST.2022.3149272.

\bibitem{energy-consumption-control} M. Stoyanova, Y. Nikoloudakis, S. Panagiotakis, E. Pallis, and E. K. Markakis, “A Survey on the Internet of Things (IoT) Forensics: Challenges, Approaches, and Open Issues,” IEEE Commun. Surv. Tutorials, vol. 22, no. 2, pp. 1191–1221, 2020, doi: 10.1109/COMST.2019.2962586.

\bibitem{iot-forensics-survey} M. Stoyanova, Y. Nikoloudakis, S. Panagiotakis, E. Pallis, and E. K. Markakis, “A Survey on the Internet of Things (IoT) Forensics: Challenges, Approaches, and Open Issues,” IEEE Commun. Surv. Tutorials, vol. 22, no. 2, pp. 1191–1221, 2020, doi: 10.1109/COMST.2019.2962586.

\bibitem{future-chlg} Majid M, Habib S, Javed A R, et al. Applications of wireless sensor networks and internet of things frameworks in thISACe industry revolution 4.0: A systematic literature review[J]. Sensors, 2022, 22(6): 2087.

\bibitem{sniffer} X. Guo, T. Gao, C. Dong, K. Cao, Y. Nan and F. Yu, "A Real-time Network Monitoring Technique for Wireless Sensor Networks," 2022 IEEE 12th International Conference on Electronics Information and Emergency Communication (ICEIEC), 2022, pp. 32-36, doi: 10.1109/ICEIEC54567.2022.9835059.

\bibitem{mac-protocol} Dong C, Yu F. An efficient network reprogramming protocol for wireless sensor networks[J]. Computer Communications, 2015, 55: 41-50.

\bibitem{mtnblt-sw} H. Alsolai and M. Roper, “A systematic literature review of machine learning techniques for software maintainability prediction,” Information and Software Technology, vol. 119, p. 106214, Mar. 2020, doi: 10.1016/j.infsof.2019.106214.

\bibitem{mtnblt-mech} X. Luo, Z. Ge, S. Zhang, and Y. Yang, “A method for the maintainability evaluation at design stage using maintainability design attributes,” Reliability Engineering \& System Safety, vol. 210, p. 107535, Jun. 2021, doi: 10.1016/j.ress.2021.107535.

\bibitem{mtnblt-IE}	S. Ahmadi, S. Moosazadeh, M. Hajihassani, H. Moomivand, and M. M. Rajaei, “Reliability, availability and maintainability analysis of the conveyor system in mechanized tunneling,” Measurement, vol. 145, pp. 756–764, Oct. 2019, doi: 10.1016/j.measurement.2019.06.009.

\bibitem{zqc} Q. Zhang, C. Dong and F. Yu, "Maintenance of Large Scale Wireless Sensor Networks," 2022 IEEE 5th International Conference on Electronics Technology (ICET), 2022, pp. 929-932, doi: 10.1109/ICET55676.2022.9825017.

\bibitem{sj} Shen J, Qiu C, Yu F. A Maintainability Evaluation Method for Wireless Sensor Networks Based on AHP and Fuzzy Comprehensive Evaluation[C]//2019 IEEE 2nd International Conference on Electronics and Communication Engineering (ICECE). IEEE, 2019: 143-147.

\bibitem{gtn} T. Gao and F. Yu, "A Maintainability Evaluation Method of Large Scale Wireless Sensor Networks Based on Sample Entropy," 2022 IEEE 12th International Conference on Electronics Information and Emergency Communication (ICEIEC), 2022, pp. 37-41, doi: 10.1109/ICEIEC54567.2022.9835079.

\bibitem{qct} Qiu C, Shen J, Yu F. A Maintainability Estimation Method for Wireless Sensor Networks[C]//2019 IEEE 5th International Conference on Computer and Communications (ICCC). IEEE, 2019: 604-608.

\bibitem{wc} C. Wang, X. Guo and F. Yu, "Maintenance Study Based on Bayesian Network and Expectation-Maximum Algorithm," 2022 IEEE 12th International Conference on Electronics Information and Emergency Communication (ICEIEC), 2022, pp. 27-31, doi: 10.1109/ICEIEC54567.2022.9835032.


\bibitem{x-ai} Montavon G, Kauffmann J, Samek W, et al. Explaining the predictions of unsupervised learning models[C]//International Workshop on Extending Explainable AI Beyond Deep Models and Classifiers. Springer, Cham, 2022: 117-138.

\bibitem{serverless-computing} Li Y, Lin Y, Wang Y, et al. Serverless Computing: State-of-the-Art, Challenges and Opportunities[J]. IEEE Transactions on Services Computing, 2022.

\bibitem{gill2022ai} Gill S, Xu M, Ottaviani C, Patros P, Bahsoon R, Shaghaghi A, Golec M, Stankovski V, Wu H, Abraham A and Singh M. "AI for next generation computing: Emerging trends and future directions," Internet of Things, Vol. 19, p. 100514, 2022.

\bibitem{XuCSUR2022}  Zhong X, Xu M, Rodriguez A, Xu C, Buyya R. "Machine learning-based orchestration of containers: A taxonomy and future directions." ACM Computing Surveys, Vol. 54, Iss. 10, pp. 1-35, Jan 2022

\bibitem{sc-application} S. K. Mondal, R. Pan, H. M. D. Kabir, T. Tian, and H.-N. Dai, “Kubernetes in IT administration and serverless computing: An empirical study and research challenges,” J Supercomput, vol. 78, no. 2, pp. 2937–2987, Feb. 2022, doi: 10.1007/s11227-021-03982-3.

\bibitem{HAL} Yoo S, Jerraya A A. Introduction to hardware abstraction layers for SoC[M]//Embedded software for SoC. Springer, Boston, MA, 2003: 179-186.

\bibitem{cooja} Velinov, Aleksandar, and Aleksandra Mileva. "Running and testing applications for Contiki OS using Cooja simulator." (2016): 279-285.

\end{thebibliography}

